Learning Stable Dynamical Systems for Visual Servoing

This work presents the dual benefit of integrating imitation learning techniques, based on the dynamical systems formalism, with the visual servoing paradigm. On the one hand, dynamical systems allow to program additional skills without explicitly coding them in the visual servoing law, but leveraging few demonstrations of the full desired behavior. On the other, visual servoing allows to consider exteroception into the dynamical system architecture and be able to adapt to unexpected environment changes. The beneficial combination of the two concepts is proven by applying three existing dynamical systems methods to the visual servoing case. Simulations validate and compare the methods; experiments with a robot manipulator show the validity of the approach in a real-world scenario.

==> Sections/RelatedWork.tex <==
\section{Related Work}\label{sec:rel_work}

\todo{I think we can remove this Section II.}

\subsection{Visual servoing}

\subsection{Skills representation using \acp{ds}}\label{sec:batch_ds_learn}
%The dynamic movement primitive (DMP) framework \cite{DMP} is one of the first examples of robotic skills representation via DS. DMPs exploit a non-linear forcing term, learned from a single demonstration, to reshape a linear dynamics, and a clock signal to suppress the non-linear force after a certain time guaranteeing the convergence towards the target. Task-parameterized motion primitives \cite{TP-DMP, Pervez18} extend the standard DMP by introducing extra task-dependent parameters useful to adapt robot movements to novel scenarios. %TP-DMP consists of a weighted summation of second order DS, learned from demonstrations using Gaussian mixture models (GMM) \cite{GMR}. 

%The stable estimator of dynamical systems (SEDS) in \cite{SEDS} generates stable motions from a non-linear DS, represented by GMM. Global stability is ensured by constraining the GMM parameters to satisfy a set of stability constraints derived from a quadratic Lyapunov function. The main advantage of SEDS is that the learned system is globally stable. The main limitation is that contradictions may occur between the demonstrations and the quadratic stability constraints, preventing an accurate learning of the desired motion.

%The accuracy problem is explicitly considered in several works \cite{NeuralLearn2, Clf, tau-SEDS, Perrin16}, showing that complex motions can be accurately represented by non-linear DS. In \cite{NeuralLearn2, Clf} two different approaches are proposed to learn a Lyapunov function which minimizes the contradictions between the stability constraints and the training data, favoring an accurate reproduction of complex motions. \cite{tau-SEDS} learns a diffeomorphic transformation that projects the training data into a space where they are well represented by a quadratic Lyapunov function. Perrin et al. \cite{Perrin16} propose a fast algorithm to learn diffeomorphic transformations from a single demonstration. % The approach considers only one demonstration and assumes a linear DS.}

%RDS is complementary to the state-of-the-art approaches for skill representation via DS. RDS, in fact, incrementally reshapes the trajectories of a given DS (original DS) without affecting its stability properties. The original DS can be either designed by an expert or learned from demonstrations using one of the the aforementioned approaches. 

%The main outcome of the work in \cite{NeuralLearn2, Clf, tau-SEDS, Cont-DS} is that complex motions can be accurately represented by non-linear DS.

%A common idea between [11] and [12] is to learn from demonstrations a Lyapunov function which minimizes the contradictions between the stability constraints and the training data. In [11], the DS is represented by an extreme learning machine (ELM) [13]. ELM parameters are learned by solving a constrained op-
%timization problem, where stability constraints are derived from the learned Lyapunov function. In SEDSII the learned Lyapunov function is used as control Lyapunov function [14] to compute, at run time, a stabilizing control input. Compared to SEDS, both SEDSII and the approach in [11] exhibit a superior reproduction accuracy. The main advantage of SEDSII is its applicability to any learning approach used to represent demonstrations as a dynamical system.

\subsection{Learning for visual servoing}
\cite{bateux2018training} trains a deep NN to perform robust (occlusions, illumination) pose estimation and generate references for a \ac{vs} control schema. 

\cite{pignat2019bayesian} uses Bayesian \acp{gmm} to learn the pixel to camera pose mapping.

\cite{jin2019robot} combines Uncalibrated \acl{vs} and ...

\cite{dometios2018vision} seems very related, check!


These papers might be of interest (to be checked): \cite{castelli2017machine}, \cite{jin2020geometric}, \cite{lampe2013acquiring}, \cite{vakanski2017imagebased}, \cite{phung2012tool}.

%Inferring way-points to help VS with complex tasks~\cite{Paolillo:icra:2020}
